Enhanced physics-constrained deep neural networks for modeling vanadium redox flow battery

Numerical modeling and simulation have become indispensable tools for advancing a comprehensive understanding of the underlying mechanisms and cost-effective process optimization and control of flow batteries. In this study, we propose an enhanced version of the physics-constrained deep neural network (PCDNN) approach [1] to provide high-accuracy voltage predictions in the vanadium redox flow batteries (VRFBs). The purpose of the PCDNN approach is to enforce the physics-based zero-dimensional (0D) VRFB model in a neural network to assure model generalization for various battery operation conditions. Limited by the simplifications of the 0D model, the PCDNN cannot capture sharp voltage changes in the extreme SOC regions. To improve the accuracy of voltage prediction at extreme ranges, we introduce a second (enhanced) DNN to mitigate the prediction errors carried from the 0D model itself and call the resulting approach enhanced PCDNN (ePCDNN). By comparing the model prediction with experimental data, we demonstrate that the ePCDNN approach can accurately capture the voltage response throughout the charge--discharge cycle, including the tail region of the voltage discharge curve. Compared to the standard PCDNN, the prediction accuracy of the ePCDNN is significantly improved. The loss function for training the ePCDNN is designed to be flexible by adjusting the weights of the physics-constrained DNN and the enhanced DNN. This allows the ePCDNN framework to be transferable to battery systems with variable physical model fidelity.

==> sections/BackupSections/Elsevier.tex <==
\section{The Elsevier article class}

\paragraph{Installation} If the document class \emph{elsarticle} is not available on your computer, you can download and install the system package \emph{texlive-publishers} (Linux) or install the \LaTeX\ package \emph{elsarticle} using the package manager of your \TeX\ installation, which is typically \TeX\ Live or Mik\TeX.

\paragraph{Usage} Once the package is properly installed, you can use the document class \emph{elsarticle} to create a manuscript. Please make sure that your manuscript follows the guidelines in the Guide for Authors of the relevant journal. It is not necessary to typeset your manuscript in exactly the same way as an article, unless you are submitting to a camera-ready copy (CRC) journal.

\paragraph{Functionality} The Elsevier article class is based on the standard article class and supports almost all of the functionality of that class. In addition, it features commands and options to format the
\begin{itemize}
\item document style
\item baselineskip
\item front matter
\item keywords and MSC codes
\item theorems, definitions and proofs
\item lables of enumerations
\item citation style and labeling.
\end{itemize}

\section{Front matter}

The author names and affiliations could be formatted in two ways:
\begin{enumerate}[(1)]
\item Group the authors per affiliation.
\item Use footnotes to indicate the affiliations.
\end{enumerate}
See the front matter of this document for examples. You are recommended to conform your choice to the journal you are submitting to.

\section{Bibliography styles}

There are various bibliography styles available. You can select the style of your choice in the preamble of this document. These styles are Elsevier styles based on standard styles like Harvard and Vancouver. Please use Bib\TeX\ to generate your bibliography and include DOIs whenever available.

Here are two sample references: \cite{Feynman1963118,Dirac1953888}.


\section*{References}


==> sections/BackupSections/backup-theory.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Numerical model & PINN %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methodology}\label{sec:method}
%
The physical models presented in this paper that describe the governing physical phenomena and reaction kinetics in the electrolytes, electrodes, and the membrane are based on the simplifications of 0D model developed in \cite{Shah2011} unless otherwise stated.
%For a vanadium redox flow battery (VRFB) cell shown in Figure. \ref{fig:sche_model}, the assumptions and simplifications used for the 0D model \cite{Shah2011} are adopted in this study unless otherwise stated.
Briefly, the 0D model is derived by lumping the variables in each component of the VRFB under isothermal operation, and concentration variation along any direction in the electrode and reservoir is negelected. 
Also, we assumed the electrolytes as a dilute solution with electro-neutrality and uniformly distributed in the porous electrodes. Each half reaction occurs in the respective electrodes, and crossover of vanadium ions through the membrane and any other side reactions are not considered in the model. Protons and water are transported through the membrane without accumulation. During a charging-discharing process, the electrolytes are circulated between the respective electrodes and reservoirs at a constant flow rate.

The knetics associated with reduction and oxidation of vanadium species are expressed as the following simplified set of half-reactions:
\begin{subequations}\label{eq:reaction}
\begin{align}
& - \text{ve electrode}: \text{V(III)} + \ce{e-} \ce{<=>} \text{V(II)}  \\
& + \text{ve electrode}:  \ce{VO^2+} + \ce{H2O} \ce{<=>} \ce{VO2+} + 2\ce{H+} + \ce{e-}
\end{align}
\end{subequations}

%%% ---------------------------------
% Numerical model
%%% ---------------------------------
\subsection{Physical model}
%
\subsubsection{Concentration computation}\label{sec:concentration}
Let $c_i, i \in \mathcal{S} = \{\text{V(II)}, \text{V(III)}, \text{V(IV)}, \text{V(V)}, \text{H}^+, \text{H}_2 \text{O}\}$ denote the concentration of active species $i$ in liquid, where the subscripts $\text{V(IV)}$ and $\text{V(V)}$ refer to \ce{VO^2+} and \ce{VO2+}, respectivly. 
For brevity, the subscripts "$n$" and "$p$" is used to denote the quantities associated with the \textit{negative} and \textit{positive} electrode, respectively. For instance, $c_{\text{H}^+_p}$ is the concentration of protons $[\ce{H+}]$ in the positive electrode.

The governing equations for solving the concentration of species $c_i$ are summarized in \ref{sec:append-concentration}, where the conservation of mass and charge, the recirculation of the electrolyte through external reservoirs, the transport of species across membrane, and the electrochemical reactions in electrodes during charge and discharge processes are considerred under the 0D model \cite{Shah2011}.
%that describe the fluid dynamic and electrochemical responses in a single-cell VRFB. 
%The concentration of the active species (i.e., $\mathcal{S}$ = \{V(II), V(III), V(IV), V(V), $\text{H}^+$, $\text{H}_2 \text{O}$\}) can be obtained by using the mass balance euqaiotns 
%\textit{The model is based on the principles of mass and charge conservation, incorporating the major resistances, the electrochemical reactions and recirculation of the electrolyte through external reservoirs. }
It is noted that with the 0D model assumption, the concentration of specie $c_i$ can be expressed as a scalar function with respect to the state of charge (SOC), i.e. $c_i = c_i(\text{SOC})$. 
Subsequently, the reaction kinetics associated with 0D VRFB model are reviewed in next subsection.

%%%%%%%%%%%%%%%%%%%%%
%
\subsubsection{Reaction kinetics}\label{sec:reaction_kinetics}
%
Following the study in~\cite{Shah2011,Sharma2015,Eapen2019,Lee2019c}, the cell voltage under investigation can be calculated from the following formula: 
\begin{equation}\label{eq:cell}
E^{cell} = E^{OCV} + \eta^{act} + \eta^{ohm}
\end{equation}
where $E^{OCV}$ is the reversible open circuit voltage (OCV), $\eta^{act}$ is the activation overpotential, and $\eta^{ohm}$ is the ohmic losses. These components will be further explained in the following.
%Given an applied current $I$, the cell voltage (or cell potential difference) should be sufficient to drive the forward reaction as well as overcome the irreversible losses. In this study, we only consider the activation and ohmic losses and ignore concentration loss because we assume the system does not undergo very high current densities. Futhermore, self discharge is neglected. 


The OCV can be approximated by using the Nernst's equation with introducing the Donnan potential arising across the membrane due to the differences in proton activities between both half-cells \cite{Knehr2011}:
%\begin{equation}\label{eq:kin_rev}
%E_{cell}^{rev} = E_2^0 - E_1^0 + \frac{RT}{F} \ln \left( \frac{c_{\text{V(II)}} c_{\text{V(V)}}}{c_{\text{V(III)}} c_{\text{V(IV)}}} \right) +
%\frac{RT}{F} \ln \left( \frac{c_{\text{H}^+,2}} { c_{\text{H}^+,1}} \right)
%+ \frac{RT}{F} \ln \left( \frac{c^2_{\text{H}^+,2}}{c_{\text{H}_2 \text{O},2}} \right)
%\end{equation}
\begin{equation}\label{eq:kin_rev}
E^{OCV} = E_p^0 - E_n^0 
+ \frac{RT}{F} \ln \left( \frac{c_{\text{V(II)}} c_{\text{V(V)}} c_{\text{H}^+_p} c^2_{\text{H}^+_p}}
{c_{\text{V(III)}} c_{\text{V(IV)}}   c_{\text{H}^+_n}  c_{\text{H}_2 \text{O}_p} } \right)
\end{equation}
where $c_i \: (i \in \mathcal{S} = \{\text{V(II)}, \text{V(III)}, \text{V(IV)}, \text{V(V)}, \text{H}^+, \text{H}_2 \text{O}\})$ are the concentration of species obtained by using the 0D model \cite{Shah2011} introduced in Section \ref{sec:concentration} and \ref{sec:append-concentration}), and $E_n^0$ and $E_p^0$ are the negative and postive equilibrium potentials under the standard condition, respectively. Since protons in the positive electrolyte is undergoing a redox reaction to form water, the proton-water redox couple is also considered in Eq. (\ref{eq:kin_rev}). The consideration of water concentraion helps to reduce the OCV discrepancy compated to experimental observation \cite{Eapen2019}.


The activation overpotential in Eq. (\ref{eq:cell}) is described by Butler-Volmer equations~\cite{newman2012electrochemical}. Here, assuming the equal transfer coefficient is $0.5$ for both electrodes and the reaction rate constant remains the same for both reduction and oxidation~\cite{Shah2011,Eapen2019}, $\eta^{act}$ is expressed as:
\begin{equation}\label{eq:eta_act}
\eta^{act} = |\eta_{n}| + |\eta_{p}|
\end{equation}
\begin{equation}\label{eq:eta_neg}
\eta_{n} = -\frac{2RT}{F} \arcsinh \left( \frac{j}{2Fk_n \sqrt{c_{\text{V(II)}} c_{\text{V(III)}} }} \right) 
\end{equation}
\begin{equation}\label{eq:eta_pos}
\eta_{p} = \frac{2RT}{F} \arcsinh \left( \frac{j}{2Fk_p \sqrt{c_{\text{V(IV)}} c_{\text{V(V)}} }} \right)
\end{equation}
where $j$ is the (local) current density calculated from $j=I/A_s$ with $A_s = S V_e$, and $k_n$ and $k_p$ are the standard rate constants associated with the reactions at the positive and negative electrodes, respectively. It is worthwhile to point out that the reaction constants are temperature dependent~\cite{Shah2011}.
%that are temperature dependent, expressed as follows
% Arrhenius eqaution. F * E is assumed to be activation energy? Need to check wheter negtaive equation exact in Eapen_2019. Wrong k_1 with sign in Eapen's paper
%\begin{equation} \label{eq:k1}
%k_{1} = k_{1,ref} \exp \left( - \frac{ F E_1^0 (T_{ref})}{R} \left[\frac{1}{T_{ref}} - \frac{1}{T}\right] \right)
%\end{equation}
%\begin{equation} \label{eq:k2}
%k_{2} = k_{2,ref} \exp \left( \frac{F E_2^0 (T_{ref})}{R} \left[\frac{1}{T_{ref}} - \frac{1}{T}\right] \right)
%\end{equation}
%where $k_{1,ref}$ and $k_{2,ref}$ are the reference rate constant for the reactions in Eqs. (\ref{eq:reaction}a) and (\ref{eq:reaction}b) at $293$ K, respectively.


The ohmic losses~\cite{Shah2011,Sharma2015} associated with the current collector (c), membrane (m) and the electrolyte (e) can be expressed as follows:
\begin{equation}\label{eq:ohm}
\eta^{ohm} = \left(\frac{2w_c}{\sigma_c} + \frac{w_m}{\sigma_{m}} + \frac{2w_e}{\sigma_e^{eff}}\right) j_{app}
\end{equation}
where $j_{app} $ is the \textit{nominal} current density defined by $j_{app} = I/A_e$, and $w_c$, $w_m$ and $w_e$ are the width of the collectors, membrane and the electrodes, respectively, as illustrated in Figure \ref{fig:sche_model}. The Bruggeman correction~\cite{Bird2002} has been used in the effective conductivity of porous electrode, given by $\sigma_e^{eff} = (1-\epsilon)^{3/2} \sigma_s$.
Note that conduction in collectors and electrodes is related to the movement of electrons, whereas it is due to the movement of prontons in the membrane. Assuming a fully saturated Nafion membrane~\cite{Zawodzinski1993}($\lambda = 22$), the conductivity of membrane $\sigma_m$ is expressed by the following empirical relationship~\cite{Springer1991}:
\begin{equation}\label{eq:sigm_m}
\sigma_m = (0.5139 \lambda - 0.326) \exp \left(1268 \left[ \frac{1}{303} - \frac{1}{T} \right]\right)
\end{equation}
The default model parameters used for Equations (\ref{eq:kin_rev})-(\ref{eq:sigm_m}) are presented in Table \ref{table:parameters_model}.
%In this study, the conductivity $\sigma_e$ is a fitting parameter to be determined, .

\begin{table}[htb]
	\centering
	\small
	\caption{\textcolor{blue}{Default values for the electrochemical parameters and conductivities used in the model. (All values are in SI units).}}
%	\resizebox{\columnwidth}{!}{}
%	 \resizebox{1.0\textwidth}{!}{\begin{minipage}{\textwidth}
%\end{minipage}}
\scalebox{0.8}{
	\begin{tabular}{cccc}
		\toprule
		Parameters & Values  \\
		\hline
		Positive electrode potential, $E_p^0$      &   $1.004$   \\
		Negative electrode potential, $E_n^0$      &  $-0.26$   \\	
		Standard rate constant at $T = 293$     &  \\
		\bottomrule
	\end{tabular}
	}
	\label{table:parameters_model}
\end{table}


\begin{table}[htb]
	\centering
	\small
	\caption{\textcolor{blue}{Default values for the structural and geometric parameters used in the model (All values are in SI units).}}
	%	\resizebox{\columnwidth}{!}{%}
	\begin{tabular}{cccc}
		\toprule
		Parameters & Values  & Parameters   & Values  \\
		\hline
		Temperature, $T$     & $293$    & $1.676 \times 10^{-3}$     & $1.959 \times 10^{-2}$   \\		
		\multicolumn{1}{c}{$3 \times 50$}      & $8.059 \times 10^{-4}$    & $1.218 \times 10^{-3}$     & $1.957 \times 10^{-2}$   \\	
		%			\hline
		\multicolumn{1}{c}{$4 \times 30$}      & $7.770 \times 10^{-4}$    & $5.854 \times 10^{-4}$     & $1.950 \times 10^{-2}$   \\	
		%		\multicolumn{1}{c}{$4 \times 40$}      & $6.075 \times 10^{-4}$    & $8.917 \times 10^{-4}$     & $1.951 \times 10^{-2}$   \\	
		\multicolumn{1}{c}{$4 \times 50$}      & $5.843 \times 10^{-4}$    & $6.381 \times 10^{-4}$     & $1.951 \times 10^{-2}$   \\	
		\bottomrule
	\end{tabular}%
	\label{table:Geometries}
\end{table}

%\begin{table}[htb]
%	\centering
%	\small
%	\caption{Default values for the electrochemical parameters and conductivities used in the model. (All values are in SI units).}
%	%	\resizebox{\columnwidth}{!}{%}
%	\begin{tabular}{cccc}
%		\toprule
%		Parameters & Values  & Parameters   & Values  \\
%		\hline
%			Reference temperature, $T$     & $7.956 \times 10^{-4}$    & $1.676 \times 10^{-3}$     & $1.959 \times 10^{-2}$   \\		
%		Positive electrode potential, $E_p^0$      &   $1.004$  & $9.186 \times 10^{-3}$     & $2.019 \times 10^{-2}$   \\
%		Negative electrode potential, $E_n^0$      &  $-0.26$     & $4.152 \times 10^{-3}$     & $2.652 \times 10^{-2}$   \\	
%		Reference temperature, $T$     & $7.956 \times 10^{-4}$    & $1.676 \times 10^{-3}$     & $1.959 \times 10^{-2}$   \\		
%		\bottomrule
%	\end{tabular}%
%	\label{table:operating_conditions}
%\end{table}

%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Model prediction \& parameters}
%
The overall voltage of the investigated VRFB is calculated using Equations ... All the operating parameters and property values used in this study are listed in Table 1.
In 0D model, 
Usually, calibrated 0D model will be used for ... for example, the 0D prediction use the following 

Although many studies have demonstrated that 0D model were capbable of predicting the dynamic changes of the cell voltage output under different operating conditions [], the characterization of the associated lumped parameters remains elusive. Previous studies mainly relied on fitting the parameters with respect to certain specific experimental observation and thus lack of generalization [].

All the averaged concentrations are estimated according to the state of charge (SOC) and, for discharging, are calculated using Eq. (8). 

\textcolor{blue}{As pointed out in (Choi et al., 2020), the surface concentrations is related to the local mass flux of the species at the surface and influnced by the flow velocity.}
Moreover, 
as pointed out in~\cite{Shah2008,Chen2014a,Tang2014,Murthy2018}, the surface concentrations is related to the local mass flux of the species at the surface and influnced by the flow velocity.
\subsubsection{Operating conditions}
In this study, we consider $mathcal{P}={u, I, c^0_V}$


As shown in Figure XX (from the study in 0D model [references]), the 0D model is able to predict the experimental test with the model parameter...
is limited to the construction of lumped parameter model, and the associated parameter fitting is usually task specific and complicated.


%%% ---------------------------------
% MPINN
%%% ---------------------------------
\subsection{Physics-informed neural networks (PINNs)}
%
In this study, we propose to use the PINN approach to estimate model parameters from the given experimental data (e.g., SOC–V curve). Different from other pure data-driven neural networks scheme,  the prediction of cell voltage prediction is obtained through a predefined physical model with undetermined model parameters rather than directly learning the mapping from the inputs to the voltage outputs. The employment of the well-established physical model prevents the unstable voltage prediction that usually occurs in deep neural netwrok (DNN) approach; (besides, it provides meaningful parameter characterization ...)

In addition, because the prediction of PINN model is limited to the underlying physical model, it is incapable to capture complex charging-discharging behavior related to the tail or concentration overpotential. To achieve a better voltage prediction, we equipped the PINN with a addtional neural network enhancements, called multifidelity PINN (MPINNs)


To enhance the adaptability and generalization of the developing digital twin model, we propose a physics-informed deep neural network (PINN) framework that integrates both the well established physical models and the data-driven approach with available data. This novel PINN framework aims to construct a deep learning model for automated calibration of model parameters and improved prediction for a wide range of process conditions including applied current, inlet flow rate, and initial concentration. 

In this study, we propose to use physics-informed neural networks (PINNs) to identify the model parameter with respect to various operting conditions of the VRFB system. For demonstration, we consider the inlet velocity $\tilde{u}$, applied current $I$, and the initial concentration 

%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Preparation of measurement data}
%

In the present study, we use voltage curves (E) obtained 

time is converted to SOC using 0D analytical soltution..in Appendix.

The proposed PINN approach is used to

\textit{In the present PI method, we use voltage curves (Vobs) obtained from experiments (or reference simulations) for a specific RFB system to identify the parameters of the numerical model described in Section 2.1.}

each experiments associated with one set of operation conditions

[1] S. B. Lee et al., “Open data, models, and codes for vanadium redox batch cell systems: A systems approach using zero-dimensional models,” J. Electrochem. Energy Convers. Storage, vol. 17, no. 1, 2019.

%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Physics-informed neural networks (PINNs) for parameter identification}\label{sec:pinn}
% Describe how to use PINN to do parameter estimation 
%
\begin{figure}[ht!]
	\centering
	\includegraphics[angle=0,width=5in]{figures/MPINN-VFB}
	\caption{Schematic of the proposed multifidelity physics-informed neural network (MPINN) model that consist of two components: the physics-informed neural networks (PINN, in the blue dashed box) and the high-fidelity DNN (in the red dashed box). In the PINN component, the $m$ identifiable parameters $\{\mu_i\}_{i=1}^m$ associated with the given physics-based electrochemical model (denoted as $\mathcal{M}$) are related with the $p$ operating conditions through 
	associated with the given   $\{x_i\}_{i=1}^p$ denotes the $p$ operating conditions as inputs to the PINN model, $\mathcal{M}$ indicates a predefined physical model used to compute species concentration, open circuit voltage, overpotentials, and ohmic losses (e.g. 0D model is used in this study).} 
	\label{fig:sche_mpinn}
\end{figure}

The PINN approach is illustrated in the left part of Figure \ref{fig:sche_mpinn} (within the blue dashed box). As pointed out before, the parameters $\vec{\mu} = (S, k_n, k_p, \sigma_e)$ associated with the given 0D model are selected as the $m=4$ identifiable parameters in this study. This choice is based on the observation in the study \cite{Choi2020} where it shows that the voltage prediction has high sensitivity to these parameters. 
\textcolor{blue}{Lee paper also find parameters k1 and k2}
%However, it is worthy of noting that the proposed PINN approach is a general approach that can be used for more identifable simultaneously. But for simplicity, we use the current setting. 

Let the model parameters $\vec{\mu}$ be a function of the operating conditions $\vec{x}$, we can use DNNs to approximate each parameter $\mu_i$, respectively, expressed as:
\begin{equation}
\mu_i (\vec{x}) \approx \hat{\mu}_i (\vec{x}; \theta_i) = \mathcal{NN}(\vec{x};\theta_i),  \quad \text{for} \;  i = 1,...,m
%\mu_i  \in  \{S, k_1, k_2, \sigma_e\}
\end{equation}
where $\mathcal{NN}$ denotes a DNN model with the trainable weight coefficients $\theta_i$, $\vec{x}$ is a vector composed of $p$ operating conditions of interest. In this study, we consider the velocity $u$, applied current $I$, and the intial vanadium concentration $c^0_V$ as the operating conditions, thus, $\vec{x}=(u, I, c^0_V)$. We refere the interested readers to the \ref{sec:DNN-appr} for the brief review of the fully-connected feed-forward network architecture used in this study.

With the model parameters $\hat{\vec{\mu}}(\vec{x}) = (\hat{S}(\vec{x}), \hat{k}_n(\vec{x}), \hat{k}_p(\vec{x}), \hat{\sigma}_e(\vec{x}))$ represented by DNNs, the physics-based electrochemical model can be used to predict cell voltage in terms of different operating conditions and SOC. That is, Eq. \ref{eq:cell} is rewritten as:
\begin{equation}\label{eq:cell_pinn}
E^{cell}_{\mathcal{M}}(\hat{\vec{\mu}}) = E^{OCV}_{\mathcal{M}} + \eta^{act}_{\mathcal{M}}(\hat{\vec{\mu}}) + \eta^{ohm}_{\mathcal{M}}(\hat{\vec{\mu}})
\end{equation}
in which the identifable model parameters $\hat{\vec{\mu}} = (\hat{S}, \hat{k}_1, \hat{k}_2, \hat{\sigma}_e)$  are used in computing the activation overpotential $\eta^{act}_{\mathcal{M}}$ and the ohmic losses $\eta^{ohm}_{\mathcal{M}}$ defined in Eqs. (\ref{eq:eta_act})- (\ref{eq:ohm}), whereas the reversible open circuit voltage $E^{OCV}_{\mathcal{M}}$ is independent of the selected model parameters and thus it is not associated with $\hat{\vec{\mu}}$. In Eq. (\ref{eq:cell_pinn}), the subscript $\mathcal{M}$ denotes the given physical model (i.e., 0D model in this study) used to compute concentrations and different voltage components in the PINN approach. 
%the parameters $\vec{\mu} = (S, k_1, k_2, \sigma_e)$ with default values used to obtain are replaced by $\hat{\vec{\mu}} = (\hat{S}, \hat{k}_1, \hat{k}_2, \hat{\sigma}_e)$ with the DNN weights $\{\theta_i\}_{i=1}^{m}$ to be determined. But note that 
% in both Eqs. (\ref{eq:kin_rev}) and (\ref{eq:cell_pinn})
% In calculating $E^{OCV}$ and $\eta^{act}(\hat{\vec{\mu}})$, 
% Concentration
According to the derivation in \ref{sec:append-concentration}, all the concentrations $c_i, i \in \mathcal{S} $ used in $E^{OCV}_{\mathcal{M}}$ and $\eta^{act}_{\mathcal{M}}$ can be estimated by given the state of charge (SOC):
%Pluging $$c_{V(II)}$ in Eq. (\ref{})
\begin{equation}\label{eq:SOC_pinn}
\left\{
\begin{array}{ll}
\begin{split}
& c_{\text{V(II)}}  = c_{V}^0 \times \text{SOC} \\
& c_{\text{V(III)}} = c_{V}^0 \times (1-\text{SOC}) \\
& c_{\text{V(IV)}} = c_{V}^0 \times (1-\text{SOC}) \\
& c_{\text{V(V)}}  = c_{V}^0 \times \text{SOC} \\
& c_{\text{H}^+_n}  = c_{\text{H}^+_n}^0 + c_{V}^0 \times \text{SOC} \\
& c_{\text{H}^+_p}  = c_{\text{H}^+_p}^0 + c_{V}^0 \times \text{SOC} \\
& c_{\text{H}_2 \text{O}_p}  = c_{\text{H}_2 \text{O}_p} - (1 + n_d) c_{V}^0 \times \text{SOC}
\end{split}
\end{array} \right.
\end{equation}
where $c_{V}^0 = c_{V_p}^0 = c_{V_p}^0$ is the totoal vanadium concentration specified for the negative and positive electrodes, the terms $c_{\text{H}^+_n}^0$ and $c_{\text{H}^+_p}^0$ are the initial proton concentration in the negative and positive electrodes, and $c_{\text{H}_2 \text{O}_p}$ is the intial water concentration in the positive electrode. 

Using the predicted voltage $E^{cell}_{\mathcal{M}}(\vec{c};\hat{\vec{\mu}}(\vec{x}))$ computed by Eqs. (\ref{eq:cell_pinn}) and (\ref{eq:SOC_pinn}) for a given SOC and operating conditions $\vec{x}=(u, I, c^0_V)$ and considering the mean square error of the voltage, we define a loss (or objective) function with the measurements $E^*(t,\vec{x})$ as follows:
%
\begin{equation}\label{eq:loss_pinn}
\mathcal{L}_{\mathcal{M}} (\vec{\theta}) = \frac{1}{N^{x}} \sum_{q=1}^{N^{x}} \frac{1}{N^t_q} \sum_{l=1}^{N^t_q} [E^{cell}_{\mathcal{M}}(t_l;\hat{\vec{\mu}}(\vec{x}_q; \vec{\theta})) - E^*(t_l,\vec{x}_q)]^2
\end{equation}
%i.e., $\vec{x}_q, q=1,...,N^x$, 
%$\vec{\theta} = \{\theta_i\}_{i=1}^m$
\textcolor{blue}{"for simpicity, denoted as $E^{cell}_{\mathcal{M}},q(\theta)$"}
where $\vec{\theta} = \{\theta_1,...,\theta_m\}$ denotes the weights in all the DNN models,  $N^x$ is the number of experiments associated with different sets of operation conditions, $N^t_q$ is the total number of data points in the SOC-V (or time-V) curves associated with the operating conditions $\vec{x}_q$, and the index $l$ denotes a data point having different SOC or time values. \textcolor{blue}{Note that the time and SOC is related by using Eq ()}. If we denote a new array $\vec{z} = (t, \vec{x})$ to encode both the time variable $t$ and the input conditons $\vec{x}$, the loss function in Eq. (\ref{eq:loss_pinn}) is simplified as:
% ref to Lee et al. (2019) open data...; Choi et al. (2020)
\begin{equation}\label{eq:loss_pinn2}
\mathcal{L}_{\mathcal{M}} (\vec{\theta}) = \frac{1}{N} \sum_{n=1}^{N}  [E^{cell}_{\mathcal{M}}(\vec{z}_n) - E^*(\vec{z}_n)]^2
\end{equation}
where $N$ is the total number of the measured data points used for training the DNN weight coefficients $\vec{\theta} = \{\theta_i\}_{i=1}^m$. The optimal solution is defined as $\hat{\vec{\theta}}$. 
 
\textcolor{blue}{...L-BFGS-B...}
After training to obtain the optimal weigth coefficient, the

\subsubsection{High-fidelity correction}
% Describe how to enhance prediction capacity
In Section \ref{sec:pinn}, the parameter estimation method by PINN was introduced. With the optimized parameters learned from the measurment, the PINN model leads to enhanced voltage prediction $E_{\mathcal{M}}^{cell}$. 
Although the 0D model with enhanced calibrated model parameters by the PINN approach results in  as evident by the comparative study in \textcolor{blue}{Section XX} 

Nevertheless, although the lumped models has been enhanced by the PINN approach with enhanced calibrated parameters, it is not comprehensive enough to capture the whole charging-discharge behaviours due to the \textcolor{blue}{XXX} .... Therefore, we introduce an addtional neural network to correct the original PINN prediction, coined as high-fidelity correction. In contrast, we called the PINN prediction based on 0D model as the low-fidelity model.

The idea of the high-fidelity correction is we introduce an additional DNN function $y_H(\theta_H)$ to minimize the mismatch between the low-fidelity solution $E^{cell}_{\mathcal{M}}$ and the given experimental measurements $E^*$, that is, minimizing the following loss function:
\begin{equation}\label{eq:loss_correction}
\mathcal{L}_{H} (\theta_H)  = \frac{1}{N} \sum_{n=1}^{N}  [(E^{cell}_{\mathcal{M}}(\vec{z}_n) + y_H(\vec{z}_n))- E_H^*(\vec{z}_n)]^2
\end{equation}
where the notations $N$ and $\vec{z}$ were defined in Eq. (\ref{eq:loss_pinn2}). Note that here the measurements $E_H^*$ are associated with the subscript "$H$", denoting that the data are used for training the high-fidelity correction DNN $y_H(\theta_H)$. The data set in principle can be different from $E^*$ used in Eq. (\ref{eq:loss_pinn2}), but we use the same data set in this study.

As can be seen in Eq. (\ref{eq:loss_correction}), the PINN model $E^{cell}_{\mathcal{M}}$ is also involved in the computation. If one has trained the optimal weights $\hat{\vec{\theta}}$ based on Eq. (\ref{eq:loss_pinn2}), the PINN prediction $E^{cell}_{\mathcal{M}}(\vec{z}_n;\hat{\vec{\theta}})$ can be directly with the optimal weights. However, our numerical study shows that by simultaneously learn the weights $\vec{\theta}$ for $\vec{\mu}$ and $\theta_H$ for $y_H(\theta_H)$ can yiedl higher accuracy for the PINN model. Thus, we define a total loss function:
\begin{equation}\label{eq:loss_MPINN}
\mathcal{L}  = \mathcal{L}_{\mathcal{M}} + \mathcal{L}_{H} (\theta_H)  = \frac{1}{N} \sum_{n=1}^{N}  [(E^{cell}_{\mathcal{M}}(\vec{z}_n) + y_H(\vec{z}_n))- E_H^*(\vec{z}_n)]^2
\end{equation}

%with  weights $\vec{\theta} = \{\theta_1,...,\theta_m\}$ involved in the computation needs to be solved. 
One way to solve 

There are two approaches to 

high-fidelity 

and denotes the measurements for training 

$E^{cell}_{\mathcal{M}}$ are 

%\begin{equation}\label{eq:loss_correction}
%\mathcal{L}_{H} (\theta_H) = \frac{1}{N^{x}} \sum_{q=1}^{N^{x}} \frac{1}{N^t_q} \sum_{l=1}^{N^t_q} [E^{cell}_{\mathcal{M}}(t_l;\hat{\vec{\mu}}(\vec{x}_q)) - E^*(t_l,\vec{x}_q)]^2
%\end{equation}


\begin{equation}\label{eq:loss_correction}
\mathcal{L}  = \mathcal{L}_{\mathcal{M}} + \mathcal{L}_{H} (\theta_H)  = \frac{1}{N} \sum_{n=1}^{N}  [(E^{cell}_{\mathcal{M}}(\vec{z}_n) + y_H(\vec{z}_n))- E_H^*(\vec{z}_n)]^2
\end{equation}

where the notations $N$ and $\vec{z}_n$ are defined in Eq. (\ref{eq:loss_pinn2}), and $E^{cell}_{\mathcal{M}}$ are $E_H^*$ denotes the measurements for 
but it is physics-agnostic


\textcolor{blue}{...continue...}

\textit{The lumped models served chiefly as monitoring and control tools for the VRFB system but they were not comprehensive enough to be employed in the cell design and optimization. Several lumped dynamic VRFB models employed in the past were capable of predicting the dynamic changes of the cell voltage output as well as the active species concentration under different operating conditions [14,15]. }
Although 0D model provided efficient prediction with negligible cost, its predictive accuracy 



\subsubsection{Numerical details}
The procedure used in this study is as follows

\textcolor{blue}{...providing table to summary the comparative methods...}

\subsection{Parameter identification with PINNs}
% Loss equation. I should mentioned the analytical formed is exactly satisfied but in principal any PDE equaitons can be introduced into the loss function, refer to other PINN papers. 

[2020Choi] shows that not all the sensitive parameter to be included in the identified parameters.
\textit{In the present study, the identifiable parameters are denoted by ’I’. The unidentifiable pa- rameters (the specific surface area and conductivity of electrode) are denoted by ’U’ in Table 6, which are excluded from the best subset and specified with the reference values in the literature. It is worthy to note that parameters with high overall sensitivity do not necessarily have to be included in the best subset to be identified, while the effects of un- identifiable parameters on the model output appear to be correlated with other parameters.}



\subsection{Data Availability}
The data that support the findings of this study are available from the corresponding author upon reasonable request.

==> sections/BackupSections/outline.tex <==
\section{Outline}

\emph{Goal}: The present PI method consists of three major parts: 
%\begin{enumerate}[(1)]
%	\item obtaining a voltage curve via numerical simulations using the PDE model for the given parameters
%	\item obtaining FIM for finding the best subset of model parameters and calculating the confidence interval for identified pa- rameters and
%	\item finding an optimal set of parameters using the GA. 
%\end{enumerate}

%\emph{Applications}:
%\begin{enumerate}[(1)]
%	\item start with example Laplace Equation shown in Meet et al. (2020)
%	\item 1. Examples: show using CxPINN, better deal with EBC. Data assimilation 
%	\item forward problem (advection domainated)
%	\item Inversed problems
%	\item 	Cite high-speed paper, using CoxPINN I can address this problem.
%\end{enumerate}
%
%% --- Idea ---
%\textit{In this paper, we explicitly cast multi-task learning as multi-objective optimization, with the overall objective of finding a Pareto optimal solution.}
%\textit{We therefore propose an upper bound for the multi-objective loss and show that it can be optimized efficiently. }
%\textit{We further prove that optimizing this upper bound yields a Pareto optimal solution under realistic assumptions. }
%PINNs applied to multiple physical processes have attracted increasingly attention.

